Thermal dissipation as both the strength and weakness of matter. A material failure prediction by monitoring creep

In any domain involving some stressed solids, that is, from seismology to general engineering, the strength of matter is a paramount feature to understand. We here discuss the ability of a simple thermally activated sub-critical model, that includes the auto-induced thermal evolution of cracks tips, to predict the catastrophic failure of a vast range of materials. It is in particular shown that the intrinsic surface energy barrier, for breaking the atomic bonds of many solids, can be easily deduced from the slow creeping dynamics of a crack. This intrinsic barrier is however higher than the macroscopic load threshold at which brittle matter brutally fails, possibly as a result of thermal activation and of a thermal weakening mechanism. We propose a novel method to compute the macroscopic critical energy release rate of rupture, G_a, solely from monitoring slow creep, and show that this reproduces the experimental values within 50% accuracy over twenty different materials, and over more than four decades of fracture energy.

==> table_alpha.tex <==
\begin{table*}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|}
\cline{2-10}
                                                    & \multicolumn{1}{l|}{$\lambda$ (SI)} & \multicolumn{1}{l|}{$\phi$ (-)} & \multicolumn{1}{l|}{$V_0$ (m/s)} & \multicolumn{1}{l|}{$\alpha$ (m)} & \multicolumn{1}{l|}{$T_0$ (K)}  & \multicolumn{1}{l|}{$G_c$ (J/m$^2$)} & \multicolumn{1}{l|}{$G_a$ real (J/m$^2$)} & \multicolumn{1}{l|}{$G_a$ model (J/m$^2$)} & \multicolumn{1}{l|}{Ra (-)} \\ \hline
\multicolumn{1}{|l|}{Acrylic adhesive}              & 0.4                              & 1                            & 30                            & 2.1E-11                        & 296                          & \textbf{150}                   & \textbf{90}                        & \textbf{97}                       & 5.7                         \\ \hline
\multicolumn{1}{|l|}{Paper}                         & 0.035                            & 0.12                         & 1300                          & 2.0E-12                        & 296                          & \textbf{25390}                 & \textbf{14000}                     & \textbf{9500}                     & 15.6                        \\ \hline
\multicolumn{1}{|l|}{Bulk PMMA}                     & 0.18                             & 0.2                          & 880                           & 8.0E-12                        & 296                          & \textbf{1275}                  & \textbf{700}                       & \textbf{582}                      & 10.9                        \\ \hline
\multicolumn{1}{|l|}{Interfacial PMMA}              & 0.18                             & 0.2                          & 880                           & 2.5E-11                        & 298                          & \textbf{275}                   & \textbf{140}                       & \textbf{186}                      & 13.5                        \\ \hline
\multicolumn{1}{|l|}{HD Polyethylene}                  & 0.4                              & 0.5                          & 900                           & 7.7E-13                        & 293                          & \textbf{200000}                & \textbf{70000}                     & \textbf{87000}                    & 16.6                        \\ \hline
\multicolumn{1}{|l|}{Soda lime glass}               & \cellcolor[HTML]{ECF4FF}1        & 0.5                          & 3400                          & 1.3E-10                        & 296                          & \textbf{12}                    & \textbf{8}                       & \textbf{10}                      & 8.3                         \\ \hline
\multicolumn{1}{|l|}{Sapphire}                      & 24                               & 0.5                          & 6000                          & 7.8E-11                        & 296                          & \textbf{36}                    & \textbf{20}                        & \textbf{32}                       & 6                         \\ \hline
\multicolumn{1}{|l|}{Quartz}                        & \cellcolor[HTML]{ECF4FF}8        & 0.5                          & 3400                          & 8.8E-11                        & 293                          & \textbf{21}                    & \textbf{13}                        & \textbf{18}                       & 5.7                         \\ \hline
\multicolumn{1}{|l|}{Westerly Granite (ambient)}             & \cellcolor[HTML]{ECF4FF}2        & 0.5                          & 3000                          & 3.5E-11                        & 293                          & \textbf{120}                   & \textbf{68}                        & \textbf{92}                      & 8.5                         \\ \hline
\multicolumn{1}{|l|}{Westerly Granite (hot)}                 & \cellcolor[HTML]{ECF4FF}2        & 0.5                          & 3000                          & 8.2E-11                        & \cellcolor[HTML]{FFCCC9}573  & \textbf{43}                    & \textbf{24}                        & \textbf{35}                       & 6.8                         \\ \hline
\multicolumn{1}{|l|}{Kumamoto Andesite}                      & \cellcolor[HTML]{ECF4FF}1        & 0.5                          & 2200                          & 4.0E-11                        & \cellcolor[HTML]{FFCCC9}330  & \textbf{122}                   & \textbf{80}                        & \textbf{97}                       & 8.8                         \\ \hline
\multicolumn{1}{|l|}{Scioto Sandstone}                     & \cellcolor[HTML]{ECF4FF}2        & 0.5                          & 2000                          & 5.2E-11                        & 296                          & \textbf{55}                    & \textbf{37}                        & \textbf{44}                       & 7.3                         \\ \hline
\multicolumn{1}{|l|}{Cement paste}                        & \cellcolor[HTML]{ECF4FF}1        & 0.5                          & 2200                          & 4.2E-11                        & 298                          & \textbf{310}                   & \textbf{250}                       & \textbf{285}                      & 10.7                        \\ \hline
\multicolumn{1}{|l|}{HSULP Concrete}                      & 0.8                              & 0.5                          & 3000                          & 1.0E-10                        & 293                          & \textbf{44}                    & \textbf{38}                        & \textbf{40}                       & 9.9                         \\ \hline
\multicolumn{1}{|l|}{Vitreous carbon}               & \cellcolor[HTML]{ECF4FF}5        & 0.5                          & 2600                          & 1.6E-10                        & 296                          & \textbf{15}                    & \textbf{13}                        & \textbf{14}                       & 7.2                         \\ \hline
\multicolumn{1}{|l|}{Lead Zirconate Titanate (PZT)} & \cellcolor[HTML]{ECF4FF}1        & 0.5                          & 2000                          & 6.5E-11                        & 296                          & \textbf{40}                    & \textbf{24}                        & \textbf{33}                       & 11.3                        \\ \hline
\multicolumn{1}{|l|}{Tetragonal zirconia (TZP)}     & \cellcolor[HTML]{ECF4FF}2        & 0.5                          & 1600                          & 1.1E-11                        & 298                          & \textbf{1900}                  & \textbf{1500}                      & \textbf{1530}                     & 10.9                         \\ \hline
\multicolumn{1}{|l|}{Silicon nitride}               & \cellcolor[HTML]{DAE8FC}30       & 0.5                          & 5500                          & 3.3E-11                        & \cellcolor[HTML]{FFA19F}1573 & \textbf{510}                   & \textbf{260}                       & \textbf{400}                      & 8.9                         \\ \hline
\multicolumn{1}{|l|}{2650 T6 Aluminium alloy}               & \cellcolor[HTML]{DAE8FC}150      & 0.5                          & 3100                          & 2E-12                        & \cellcolor[HTML]{FFCCC9}448  & \textbf{54600}                 & \textbf{27000}                     & \textbf{39000}                    & 10.1                        \\ \hline
\multicolumn{1}{|l|}{AISI 310S Stainless Steel alloy}         & \cellcolor[HTML]{ECF4FF}14       & 0.5                          & 3000                          & 7.4E-13                        & 298                          & \textbf{267000}                & \textbf{101500}                    & \textbf{158500}                   & 13.4                        \\ \hline
\multicolumn{1}{|l|}{Ti-6A1-6V-2Sn Titanium}           & \cellcolor[HTML]{ECF4FF}7        & 0.5                          & 3100                          & 7.9E-13                        & 298                          & \textbf{191000}                & \textbf{72000}                     & \textbf{93000}                    & 14.9                        \\ \hline
\end{tabular}
\caption{Model parameters for various materials of the literature. The real and modelled $G_a$ thresholds are compared in the two former last columns. The cells colour help to highlight standing out value for $\lambda$ and $T_0$.}\label{table}
\end{table*}
